EmTract: Extracting Emotions from Social Media

We develop an open-source tool (EmTract) that extracts emotions from social media text tailed for financial context. To do so, we annotate ten thousand short messages from a financial social media platform (StockTwits) and combine it with open-source emotion data. We then use a pre-tuned NLP model, DistilBERT, augment its embedding space by including 4,861 tokens (emojis and emoticons), and then fit it first on the open-source emotion data, then transfer it to our annotated financial social media data. Our model outperforms competing open-source state-of-the-art emotion classifiers, such as Emotion English DistilRoBERTa-base on both human and chatGPT annotated data. Compared to dictionary based methods, our methodology has three main advantages for research in finance. First, our model is tailored to financial social media text; second, it incorporates key aspects of social media data, such as non-standard phrases, emojis, and emoticons; and third, it operates by sequentially learning a latent representation that includes features such as word order, word usage, and local context. Using EmTract, we explore the relationship between investor emotions expressed on social media and asset prices. We show that firm-specific investor emotions are predictive of daily price movements. Our findings show that emotions and market dynamics are closely related, and we provide a tool to help study the role emotions play in financial markets.

==> Tables/shap_twitter.tex <==
\begin{sidewaystable}[htbp]\centering
\caption{Shap Values: Twitter Model}\label{tab:shap_twitter}
\begin{threeparttable}
\scriptsize
\begin{tabular}{llllllllllllll}
\multicolumn{2}{c}{Neutral}  & \multicolumn{2}{c}{Happy}  & \multicolumn{2}{c}{Sad}  & \multicolumn{2}{c}{Anger} & \multicolumn{2}{c}{Disgust} & \multicolumn{2}{c}{Surprise}  & \multicolumn{2}{c}{Fear}  \\ \hline 
& & & & & & & & & & & & & \\ [\dimexpr-\normalbaselineskip+2pt]
\multicolumn{14}{l}{\textbf{Panel A: Positive Predictors}} \\
& & & & & & & & & & & & & \\ [\dimexpr-\normalbaselineskip+2pt]
backward    & 0.147 & optimism        & 0.451 & sadly         & 0.369 & frustrating & 0.375 & obama      & 0.097 & surprise     & 0.382 & scares    & 0.476 \\
scala       & 0.146 & cute            & 0.376 & weary         & 0.319 & bitter      & 0.351 & kerry      & 0.050 & curious      & 0.298 & horrific  & 0.418 \\
destination & 0.137 & joy             & 0.357 & disappointed  & 0.280 & furious     & 0.313 & nasty      & 0.048 & surprised    & 0.244 & nervous   & 0.382 \\
prefer      & 0.117 & appreciate      & 0.334 & sad           & 0.269 & temper      & 0.280 & mole       & 0.047 & confused     & 0.243 & scary     & 0.371 \\
roasted     & 0.114 & blessed         & 0.334 & disappointing & 0.225 & bastards    & 0.278 & dirty      & 0.045 & speechless   & 0.205 & fear      & 0.359 \\
hello       & 0.111 & hilarious       & 0.322 & heartbreak    & 0.216 & a**hole     & 0.271 & sg         & 0.039 & intrigued    & 0.181 & fears     & 0.349 \\
blogs       & 0.110 & excitement      & 0.320 & shame         & 0.214 & gra         & 0.201 & weird      & 0.036 & unexpected   & 0.171 & cautious  & 0.349 \\
ved         & 0.102 & loving          & 0.319 & pity          & 0.205 & p*ssed      & 0.191 & tled       & 0.035 & strange      & 0.137 & wary      & 0.349 \\
snaps       & 0.098 & congratulations & 0.291 & sorry         & 0.190 & su***       & 0.189 & presidency & 0.031 & wonder       & 0.124 & scared    & 0.312 \\
graph       & 0.095 & lovely          & 0.259 & painful       & 0.178 & burst       & 0.187 & sted       & 0.029 & doubtful     & 0.104 & panic     & 0.311 \\
inverse     & 0.093 & bliss           & 0.254 & sinking       & 0.162 & f***        & 0.185 & a**hole    & 0.029 & wondering    & 0.097 & afraid    & 0.296 \\
gles        & 0.091 & ility           & 0.245 & depressed     & 0.159 & iating      & 0.171 & awful      & 0.023 & revealed     & 0.089 & worried   & 0.277 \\
indicate    & 0.091 & laughing        & 0.241 & sma           & 0.152 & unfair      & 0.160 & greasy     & 0.022 & kidding      & 0.077 & horrible  & 0.267 \\
rental      & 0.089 & thanks          & 0.241 & failing       & 0.151 & bastard     & 0.154 & ugly       & 0.021 & unbelievable & 0.072 & nightmare & 0.262 \\
incoming    & 0.083 & cheer           & 0.239 & painfully     & 0.149 & idiot       & 0.151 & worse      & 0.020 & whoa         & 0.071 & scare     & 0.262 \\  
\multicolumn{14}{l}{\textbf{Panel B: Negative Predictors}} \\
& & & & & & & & & & & & & \\ [\dimexpr-\normalbaselineskip+2pt]
amazing     & -0.141 & bastard      & -0.077 & scala      & -0.053 & optimism        & -0.041 & panic    & -0.016 & sma         & -0.062 & p*ssed      & -0.057 \\
rt          & -0.141 & disappointed & -0.078 & nicely     & -0.053 & thankful        & -0.042 & dawn     & -0.016 & headache    & -0.062 & bliss       & -0.058 \\
terrible    & -0.151 & terrible     & -0.078 & furious    & -0.056 & curious         & -0.043 & bright   & -0.016 & hilarious   & -0.064 & bitter      & -0.058 \\
disaster    & -0.153 & horrific     & -0.080 & fears      & -0.058 & afraid          & -0.044 & dies     & -0.016 & nightmare   & -0.065 & celebrating & -0.058 \\
shaking     & -0.156 & ugly         & -0.082 & scares     & -0.059 & roasted         & -0.044 & cautious & -0.016 & sadly       & -0.067 & enburg      & -0.059 \\
optimism    & -0.156 & shame        & -0.085 & alarm      & -0.060 & blessed         & -0.047 & gui      & -0.017 & bastards    & -0.069 & ably        & -0.061 \\
cautious    & -0.158 & sadly        & -0.088 & blessed    & -0.060 & congratulations & -0.049 & pleased  & -0.018 & fears       & -0.070 & lative      & -0.062 \\
appreciate  & -0.161 & suspicion    & -0.089 & cautious   & -0.060 & loving          & -0.052 & scala    & -0.018 & horrific    & -0.071 & christmas   & -0.062 \\
cute        & -0.165 & dirty        & -0.090 & tic        & -0.063 & confused        & -0.053 & optimism & -0.018 & thankful    & -0.075 & heartbreak  & -0.074 \\
sadly       & -0.174 & fears        & -0.096 & excitement & -0.063 & scares          & -0.054 & worried  & -0.018 & blessed     & -0.078 & bastards    & -0.075 \\
horror      & -0.177 & fear         & -0.097 & temper     & -0.066 & ator            & -0.057 & surprise & -0.018 & painful     & -0.080 & surprise    & -0.078 \\
scary       & -0.178 & violated     & -0.100 & obama      & -0.069 & sober           & -0.067 & shaken   & -0.021 & weary       & -0.085 & joy         & -0.114 \\
frustrating & -0.183 & nervous      & -0.107 & surprise   & -0.072 & acle            & -0.071 & cute     & -0.024 & scares      & -0.090 & temper      & -0.119 \\
horrific    & -0.222 & frustrating  & -0.117 & bliss      & -0.092 & wary            & -0.083 & blessed  & -0.031 & frustrating & -0.095 & optimism    & -0.123 \\
headache    & -0.228 & scares       & -0.122 & savage     & -0.109 & brooke          & -0.188 & wary     & -0.033 & bitter      & -0.099 & gra         & -0.149 \\
 \hline \hline 
\end{tabular}
\begin{tablenotes}
\scriptsize 
\item Notes: Average SHAP values evaluated on 10,000 hand-tagged StockTwits messages for the Emotion Meta-Data based model. Words reported, followed by their corresponding average SHAP values, are the 15 most important words for each class. For each class separately, Panel A reports the top 15 words that are positively, while Panel B shows the top 15 words that are negatively associated with predictions. We restrict our SHAP analysis for words that appear at least 5 times in the SHAP sample. For instance, the word amazing (Panel B Column 2) is associated with a 14.1 percentage point decrease in the neutral predicted probability on average.
\end{tablenotes}
\end{threeparttable}
\end{sidewaystable}


==> Tables/trading_strategy_portfolio.tex <==
\begin{table}[htbp]\centering
\footnotesize
\begin{threeparttable}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Trading Strategy \label{tab:trading_strategy}}
\begin{tabular}{l*{8}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{Quintile 1}&\multicolumn{1}{c}{Quintile 2}&\multicolumn{1}{c}{Quintile 3}&\multicolumn{1}{c}{Quintile 4}&\multicolumn{4}{c}{Quintile 5}\\
\hline
&&&&&&&&\\[\dimexpr-\normalbaselineskip+2pt]
Mkt-RF              &     -0.0012         &      0.0330         &      0.0246         &     -0.0014         &      0.0251         &      0.0771         &     -0.0294         &      0.0090         \\
                    &    (0.0685)         &    (0.0592)         &    (0.0761)         &    (0.0574)         &    (0.0790)         &    (0.0831)         &    (0.1247)         &    (0.0606)         \\
&&&&&&&&\\[\dimexpr-\normalbaselineskip+2pt]
SMB                 &     -0.0536         &     -0.2339\sym{***}&     -0.0889         &      0.1939\sym{*}  &      0.0304         &     -0.0611         &      0.0449         &      0.0064         \\
                    &    (0.1045)         &    (0.0886)         &    (0.1267)         &    (0.1062)         &    (0.1254)         &    (0.1517)         &    (0.1916)         &    (0.0816)         \\
&&&&&&&&\\[\dimexpr-\normalbaselineskip+2pt]
HML                 &      0.1708\sym{*}  &      0.0331         &     -0.0525         &      0.0139         &     -0.2759\sym{**} &     -0.1095         &     -0.4496\sym{***}&     -0.0853         \\
                    &    (0.1015)         &    (0.0962)         &    (0.1370)         &    (0.1207)         &    (0.1125)         &    (0.1596)         &    (0.1695)         &    (0.0792)         \\
&&&&&&&&\\[\dimexpr-\normalbaselineskip+2pt]
MOM                 &      0.0127         &     -0.0222         &     -0.0469         &      0.0719         &     -0.0846         &      0.1963\sym{*}  &     -0.2609\sym{**} &      0.0073         \\
                    &    (0.0735)         &    (0.0702)         &    (0.0847)         &    (0.0816)         &    (0.0853)         &    (0.1099)         &    (0.1281)         &    (0.0600)         \\
&&&&&&&&\\[\dimexpr-\normalbaselineskip+2pt]
\alpha          &     -0.1212\sym{**} &      0.0339         &      0.1364\sym{**} &      0.1604\sym{***}&      0.2395\sym{***}&      0.0985         &      0.3843\sym{***}&      0.1982\sym{***}\\
                    &    (0.0551)         &    (0.0526)         &    (0.0587)         &    (0.0543)         &    (0.0588)         &    (0.0624)         &    (0.1025)         &    (0.0418)         \\
\hline
\hline
&&&&&&&&\\[\dimexpr-\normalbaselineskip+2pt]
Year $<$ 2016         &                     &                     &                     &                     &                     &           X         &                     &                     \\
Year $>=$ 2016        &                     &                     &                     &                     &                     &                     &           X         &                     \\
Winsorized          &                     &                     &                     &                     &                     &                     &                     &           X         \\
Observations        &   2842        &   2842        &   2842        &   2842        &   2842        &   1501        &   1341        &   2786        \\
$R^2$               &      0.0014         &      0.0022         &      0.0004         &      0.0018         &      0.0025         &      0.0048         &      0.0060         &      0.0009         \\
\hline\hline
\hline\hline
\end{tabular}
\begin{tablenotes}
\footnotesize 
\item Notes:  Robust standard errors in parentheses. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Trading strategy sorts S\&P super-composite stocks with pre-market emotion data into quintiles based on level of aggregate happiness and fear for each calendar day. The zero-cost quintile j portfolio purchases stocks in the jth quintile of investor enthusiasm, and shorts equal amount of stocks in the jth quintile of investor fear (that are not already purchased). 
\end{tablenotes}
\end{threeparttable}
\end{table}



